Attention-Guided Answer Distillation for Machine Reading Comprehension

Despite that current reading comprehension systems have achieved significant advancements, their promising performances are often obtained at the cost of making an ensemble of numerous models. Besides, existing approaches are also vulnerable to adversarial attacks. This paper tackles these problems by leveraging knowledge distillation, which aims to transfer knowledge from an ensemble model to a single model. We first demonstrate that vanilla knowledge distillation applied to answer span prediction is effective for reading comprehension systems. We then propose two novel approaches that not only penalize the prediction on confusing answers but also guide the training with alignment information distilled from the ensemble. Experiments show that our best student model has only a slight drop of 0.4% F1 on the SQuAD test set compared to the ensemble teacher, while running 12x faster during inference. It even outperforms the teacher on adversarial SQuAD datasets and NarrativeQA benchmark.

==> sections/data.tex <==
\section{Data Augmentation with Distillation}
Recently, Yu et al. \shortcite{Yu18} propose a data augmentation technique to enrich the training data by paraphrasing the passage. 
The idea is to use two translation models to translate the passage from English to another language and further translate it back into English. 
This approach helps automatically increase the amount of training data for reading comprehension tasks, resulting in a significant performance improvement.

Here we demonstrate that data augmentation can be combined with our distillation approach in a simple but effective manner. We use the ensembled teacher network to distill knowledge not only from the original training set, but also from the paraphrased data. The student is then trained on both datasets with additional soft targets. With more data and more distilled knowledge, we expect to further enhance the generalization ability of MRC models.
